Semi-supervised Learning Meets Factorization: Learning to Recommend with Chain Graph Model

Recently latent factor model (LFM) has been drawing much attention in recommender systems due to its good performance and scalability. However, existing LFMs predict missing values in a user-item rating matrix only based on the known ones, and thus the sparsity of the rating matrix always limits their performance. Meanwhile, semi-supervised learning (SSL) provides an effective way to alleviate the label (i.e., rating) sparsity problem by performing label propagation, which is mainly based on the smoothness insight on affinity graphs. However, graph-based SSL suffers serious scalability and graph unreliable problems when directly being applied to do recommendation. In this paper, we propose a novel probabilistic chain graph model (CGM) to marry SSL with LFM. The proposed CGM is a combination of Bayesian network and Markov random field. The Bayesian network is used to model the rating generation and regression procedures, and the Markov random field is used to model the confidence-aware smoothness constraint between the generated ratings. Experimental results show that our proposed CGM significantly outperforms the state-of-the-art approaches in terms of four evaluation metrics, and with a larger performance margin when data sparsity increases.

==> section/sec-experiment-three-K.tex <==
\section{Experiments}\label{experiments}

In this section, we present the comprehensive experiments that we conducted to evaluate the effectiveness of our approach.
Specifically, we compare our proposed model, i.e., RSCGM, with the state-of-the-art approaches on three real-world datasets to help us answer four key questions:
(1) How does our approach perform when comparing with the state-of-the-art approaches?
(2) How does our approach deal with the data sparsity problem?
(3) How do parameters $\lambda_F$, $\lambda_G$, and $\alpha$ affect our model performance?
(4) What is the performance difference, including running performance and prediction performance, between pairwise smoothness and joint smoothness?
(5) What is the time complexity of our approach?

\subsection{RSCGM Realizations}
Our proposed RSCGM is a generalized model to marry SSL with LFM, and we first describe  two RSCGM cases. As described in Section \hyperref[relatedwork]{\ref{relatedwork}}, there are mainly two kinds of realization of LFM in existing work. 
Thus, we apply our proposed RSCGM into both of them, i.e., a basic MF which we call it BMF \cite{mnih2007probabilistic} and a content-based MF which we call it CMF \cite{wang2011collaborative}, to evaluate the performance of RSCGM. 
%We call these two realizations BMF-RSCGM and CMF-RSCGM respectively.

BMF only uses U-I rating information, and it assumes zero mean Gaussian on user and item latent factors, i.e., $\mu_i^U=\mu_j^V=0$. In contrast, CMF assumes zero mean Gaussian on user latent factor and an item topic allocation mean Gaussian on item latent factor, i.e., $\mu_i^U=0$ and $\mu_j^V=\theta_j$, where $\theta_j$ is the topic allocation learned from item content information using topic modeling technique \cite{wang2011collaborative}.

\subsection{Experiment Settings}

We then present the datasets, baseline methods, evaluation metrics, and parameter settings during our experiments.

\stitle{Datasets.}To study how RSCGM behaves under the BMF scenario, we use hetrec2011-movielens-2k dataset (\emph{MovieLens}) \cite{cantador2011second}. 
To study how RSCGM behaves under the CMF scenario, we use hetrec2011-delicious-2k dataset (\emph{Delicious}) and dataset hetrec2011-lastfm-2k (\emph{Lastfm})\cite{cantador2011second}. These datasets, as described in Table \ref{dd}, have been popularly used  \cite{purushotham2012collaborative}.
For \emph{MovieLens}, we compute the PCC similarity \cite{ma2011recommender} between users and items to build user and item affinity graphs. 
For \emph{Delicious} and  \emph{Lastfm}, we consider the rating of a user on an item as `1' if this user has bookmarked (or listened) this item; otherwise, the user rating for the item is `0', and we take the tags of each item as its content information. 
We use the user social information to build user affinity graph, and compute the JC similarity between items to build item affinity graph, as we described in Section \hyperref[sec-energyfunction-buildgraph]{\ref{sec-energyfunction-buildgraph}}.
The densities of the U-I matrix in the three datasets are 3.97\%, 0.08\%, and 0.28\%, respectively.

\begin{table}
\scriptsize
\centering
\caption{Dataset description}
\label{dd}
\begin{tabular}{|c|c|c|c|p{1.3cm}|p{1.1cm}|}
  \hline
  Dataset & users & items & tags & user social relations & U-I ratings \\
  \hline
  \hline
  \emph{MovieLens} & 2,113 & 10,197 & -- & -- & 855,598 \\
  \hline
  \emph{Delicious} & 1,867 & 69,226 & 53,388 & 15,328 & 104,799 \\
  \hline
  \emph{Lastfm} & 1,892 & 17,632 & 11,946 & 25,434 & 92,834 \\
  \hline
\end{tabular}
\vskip -0.1in
\end{table}

%During our experiments, we split each dataset into two parts---a training dataset (80\%), and a test dataset (20\%). We train all the models on the training dataset and evaluate their performance on the test dataset.
During our experiments, we evaluate all the models using fivefold cross validation. That is, we divide each of the three dataset into five groups, and each group is used to test the rating prediction models that are learned from the other four groups.

\stitle{Baseline methods.}LFM and LFR are the state-of-the-art recommendation approaches, and thus we compare RSCGM with both LFM and LFR.
To study how RSCGM behaves under the BMF scenario, we compare our approach with the following state-of-the-art methods:
\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
	\item \textbf{IS} \cite{sarwar2001item} is an item similarity-based recommendation approach, and we use PCC to compute the similarity between items.
	\item \textbf{SSL} \cite{ding2007learning,wang2010enhanced} is a direct application of SSL, and we use it to do rating propagation on our built item affinity graph.
	\item \textbf{BMF} \cite{mnih2007probabilistic} is described in Section \hyperref[preliminary-ctr]{\ref{preliminary-ctr}}.
	\item \textbf{BMF-ULFR} \cite{ma2011recommender} adds \emph{User Latent Factor Restriction} (ULFR) on BMF, as described in Section \hyperref[preliminary-ctr]{\ref{preliminary-ctr}}.
	\item \textbf{BMF-UILFR} \cite{gu2010collaborative} adds both \emph{User and Item Latent Factor Restriction} (UILFR) on a weighted nonnegative MF approach, as described in Section \hyperref[preliminary-ctr]{\ref{preliminary-ctr}}. To make a fair comparison, we replace the weighted nonnegative MF approach with BMF.
\end{itemize}

To study how RSCGM behaves under the CMF scenario, we compare our approach with the following state-of-the-art methods, which are all side information (including item content information and user social information) aided MF:

\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
	\item \textbf{CMF} \cite{wang2011collaborative} is described in Section \hyperref[preliminary-ctr]{\ref{preliminary-ctr}}, and we do not update item topic allocation for simplification.
    \item \textbf{CMF-SMF} \cite{purushotham2012collaborative} adds user social factorization in CMF.
    \item \textbf{CMF-ULFR} \cite{chen2014context} is state-of-the-art LFR, which adds ULFR on CMF.
    \item \textbf{CMF-UILFR} \cite{gu2010collaborative} adds UILFR on a weighted nonnegative MF approach. To make a fair comparison, we also replace the weighted nonnegative MF approach with CMF.
\end{itemize}

Note that we compare with these LFMs and LFRs, not only because they are the most related models to ours, more importantly, it is because they are the state-of-the-art approaches to handle data sparsity problem in recommender systems. 

\stitle{Evaluation metrics.}Since ratings range from `1' to `5' on \emph{MovieLens}, we use Mean Absolute Error (\textit{MAE}) and Root Mean Square Error (\textit{RMSE}) to evaluate prediction performance \cite{ma2011recommender,chen2014context}:
\begin{equation}\label{mae}\small
MAE=\frac{\sum\limits_{(i,j) \in \tau}\vert{}R_{ij}-{r_{ij}}\vert{}}{|\tau|},
\end{equation}
\begin{equation}\label{rmse}\small
RMSE=\sqrt{\frac{1}{|\tau|}\sum\limits_{(i,j) \in \tau}{(R_{ij}-{r_{ij}})}^2},
\end{equation}
where $|\tau|$ is the number of predictions in the test dataset $\tau$.

Since ratings range in \{`0', `1'\} on \emph{Delicious} and \emph{Lastfm}, we use \emph{Precision} and \emph{Recall} to evaluate prediction performance \cite{sarwar2000application,wang2011collaborative,purushotham2012collaborative}. For each user, precision and recall are defined as follows:
\begin{equation}\footnotesize\nonumber
Precision@M=\frac{Number~of~items~the~user~likes~in~Top~M}{M},
\end{equation}
\begin{equation}\footnotesize\nonumber
Recall@M=\frac{Number~of~items~the~user~likes~in~Top~M}{Total~number~of~items~the~user~likes},
\end{equation}
where \emph{M} is the number of returned items. We compute the average of all the items' precision and recall in the test dataset as the final result.

\stitle{Parameter setting:}Before comparison, we use fivefold cross validation to find that BMF achieves the best performance on \emph{MovieLens} when $\lambda_U=\lambda_V=0.1$, and which we set accordingly for the rest BMF based models and RSCGM.
We also use fivefold cross validation to find that
CMF achieves the best performance on \emph{Delicious} and \emph{Lastfm} when $\lambda_U=0.01$, $\lambda_V=1$, and which we set accordingly for all the CMF based models and RSCGM. For parameter $\lambda_q$ in CMF-SMF, $\lambda_f$ in BMF-ULFR and CMF-ULFR, $\lambda$ and $\mu$ in BMF-UILFR and CMF-UILFR, and $\lambda_F$ and $\lambda_G$ in our model, we find their best values in [$10^{-3}$, $10^{-2}$, $10^{-1}$, $10^0$, $10^1$, $10^2$, $10^3$]. We also search the best value of $\alpha$ in our model in (0, 1), and we will study their effects on our model in Section \hyperref[parametereffect]{\ref{parametereffect}}.

\subsection{Comparison Results and Analysis}

%We compare our proposed model, i.e., RSCGM, with the state-of-the-art approaches on all the three dataset to prove the effectiveness of our approach.

\begin{table}\scriptsize
\centering
\caption{Performance Comparisons on \emph{MovieLens}: the smaller the better.}
\label{mf-comparison}
\begin{tabular}{|c|c|c|c|c|c|c|}
 \hline
  Metrics & \multicolumn{3}{c|}{MAE} & \multicolumn{3}{c|}{RMSE} \\
  \hline
  \hline
  IPCC & \multicolumn{3}{c|}{2.2232} & \multicolumn{3}{c|}{2.3812} \\
  \hline
  SSL & \multicolumn{3}{c|}{2.1198} & \multicolumn{3}{c|}{2.2731} \\
  \hline
  \hline
  \emph{K} & 10 & 15 & 20 & 10 & 15 & 20 \\
  \hline
  BMF & 0.6336 & 0.6316 & 0.6293 & 0.6648 & 0.6645 & 0.6639 \\ 
  \hline
  BMF-ULFR & 0.5903 & 0.5880 & 0.5858 & 0.6174 & 0.6152 & 0.6135 \\ 
  \hline
  BMF-UILFR & 0.5782 & 0.5681 & 0.5660 & 0.5992 & 0.5953 & 0.5933 \\ 
  \hline
  RSCGM & \textbf{0.5493} & \textbf{0.5485} & \textbf{0.5475} & \textbf{0.5718} & \textbf{0.5711}  & \textbf{0.5704} \\
  \hline
\end{tabular}
\vskip -0.00in
\end{table}

\begin{figure*}
\centering
%\subfigure[\emph{Delicious} K=100] { \includegraphics[width=5.5cm]{figures/lastfm100}}
%\subfigure[\emph{Delicious} K=150] { \includegraphics[width=5.5cm]{figures/lastfm150}}
%\subfigure[\emph{Delicious} K=200]{ \includegraphics[width=5.5cm]{figures/lastfm200}}\\
\subfigure[\emph{Delicious} K=100] { \includegraphics[width=5.5cm,height=4.8cm]{figures/delicious-recall-100}}
\subfigure[\emph{Delicious} K=150]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/delicious-recall-150}}
\subfigure[\emph{Delicious} K=200]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/delicious-recall-200}}\\
%\subfigure[\emph{Lastfm} K=100] { \includegraphics[width=5.5cm]{figures/lastfm-precision-100}}
%\subfigure[\emph{Lastfm} K=150]{ \includegraphics[width=5.5cm]{figures/lastfm-precision-150}}
%\subfigure[\emph{Lastfm} K=200]{ \includegraphics[width=5.5cm]{figures/lastfm-precision-200}}\\
\subfigure[\emph{Lastfm} K=100]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm-recall-100}}
\subfigure[\emph{Lastfm} K=150]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm-recall-150}}
\subfigure[\emph{Lastfm} K=200] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm-recall-200}}
\vskip -0.15in
\caption{\emph{Recall} comparison of each method on different datasets with different $M$.}
\label{ctr-compare}
\vskip -0.1in
\end{figure*}

Table \ref{mf-comparison} shows the \emph{MAE} and \emph{RMSE} comparison result on \emph{MovieLens}. 
Figure \ref{ctr-compare} shows the \emph{Recall} performance for each model on \emph{Delicious} and \emph{Lastfm}, and we omit the \emph{Precision} performance since it is similar to \emph{Recall}. We fix the parameters of each model to the best values during comparison. From it, we can see that:
\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
    \item SSL outperforms IS, since it uses smoothness insight on the item affinity graph. The rest dimensionality reduction-based methods, including RSCGM, significantly outperform SSL and IS, which shows the importance of dimensionality reduction technique.
    \item With the increase of the latent factor dimensionality $K$, the performances of all the models increase. This is because a bigger $K$ will enable us to learn a better latent factor, but it comes with the high computation complexity as a price at the same time, as we analysed in Section \hyperref[parameter-learning]{\ref{parameter-learning}}.
    \item On the dense dataset, i.e., \emph{MovieLens}, the performance difference is clear. Further observation shows that the more information the model use, the better the model performance is. This is obvious since the performance of BMF, BMF-ULFR, and BMF-UILFR increase gradually. But our model significantly outperforms BMF-UILFR (4.04\% in average), using the same information.
    \item On the sparse datasets, i.e., \emph{Delicious} and \emph{Lastfm}, CMF-SMF and CMF-ULFR slightly outperform CMF due to the additional user social information. Meanwhile, since CMF-UILFR adopts additional user and item social information, it behaves as a constant runner-up. However, LFRs' performance is limited due to their overly strong assumption that connected users or items tend to share similar latent factors. This overly strong LFR fails particularly when affinity graphs are unreliable in the data sparsity scenario, and this is why CMF-ULFR and CMF-UILFR only slightly outperforms CMF.
    \item Our model (RSCGM) consistently achieves the best performance among all the modes on all the datasets. Our approach adopts the idea of SSL, i.e., rating smoothness on the affinity graph, to alleviate the data sparsity problem, and uses a smoothness confidence decay parameter, i.e., $\alpha$, to control the rating propagation depth on the affinity graphs.
Thus, our approach always achieves the best performance even when the affinity graphs are unreliable due to the data sparsity problem.
\end{itemize}

\subsection{Data Sparsity Experiments}

To test how our approach handles the data sparsity problem, we first randomly remove some of the ratings in the U-I matrix of the original \emph{Lastfm}, and get two sub-datasets with different degree of sparsity, i.e., \emph{Lastfm20} and \emph{Lastfm50}, which mean we randomly remove 20\% and 50\% of the ratings from the \emph{Lastfm}, respectively. We then process each sub-dataset the same way as we do on the original dataset, and finally conduct contrast experiments on each of them.

\begin{figure*}
\centering
\subfigure[\emph{Lastfm20} K=100] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-precision-100}}
\subfigure[\emph{Lastfm20} K=150] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-precision-150}}
\subfigure[\emph{Lastfm20} K=200]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-precision-200}}\\
\subfigure[\emph{Lastfm20} K=100] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-recall-100}}
\subfigure[\emph{Lastfm20} K=150]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-recall-150}}
\subfigure[\emph{Lastfm20} K=200]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm20-recall-200}}\\
\subfigure[\emph{Lastfm50} K=100] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-precision-100}}
\subfigure[\emph{Lastfm50} K=150]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-precision-150}}
\subfigure[\emph{Lastfm50} K=200]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-precision-200}}\\
\subfigure[\emph{Lastfm50} K=100]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-recall-100}}
\subfigure[\emph{Lastfm50} K=150]{ \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-recall-150}}
\subfigure[\emph{Lastfm50} K=200] { \includegraphics[width=5.5cm,height=4.8cm]{figures/lastfm50-recall-200}}
\vskip -0.15in
\caption{\emph{Precision} and \emph{Recall} comparison of each method on different sparsity datasets with different $M$.}
\label{ctr-compare-sparsity}
\vskip -0.1in
\end{figure*}

Figure \ref{ctr-compare-sparsity} shows the performance for each model on different sparsity of datasets with different $K$, in which we set \emph{M} = 10, 20, 30, 40, and 50, and fix the parameters of each model to the best values. From it, we can see that:
\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
    %\item With the increase of $K$, the performance of all the models increase. This is the same reason as the comparison on \emph{Lastfm}. 
    \item With the increase of the data sparsity degree, the performance of all the models decrease. This is the standard data sparsity problem, the recommendation performance decrease with the data sparsity degree. 
    \item With the increase of the data sparsity degree, the CMF, CMF-SMF, and LFRs (CMF-ULFR and CMF-UILFR) tend to have similar performance. This is because the latent factor restriction idea fails under data sparsity scenario.
    \item Our model (RSCGM) consistently achieves the best performance among all the approaches on all the datasets. This is because of the realization of the confidence-based joint-smoothness on both $\mathcal{G}_1$ and $\mathcal{G}_2$.
    \item The sparser the dataset is, the bigger improvement of our model against the three comparison methods. Take $K=200$ for example, the average \emph{Recall} improvement of our approach over other models are 28.27\%, 35.13\%, and 48.83\% on \emph{Lastfm20} and \emph{Lastfm50} respectively. The average \emph{Precision} improvement of our approach over other models are 9.82\%, 26.12\%, and 35.58\% on \emph{Lastfm20} and \emph{Lastfm50} respectively. This is because our approach benefits from confidence-aware rating propagation we use on the affinity graphs, which alleviates the overly strong assumption of LFR.
\end{itemize}

\subsection{Compare Pairwise and Joint Smoothness}\label{smoothnesscompare}

We then study the performance difference, i.e., runtime performance (including graph build time) and prediction performance, between pairwise smoothness and joint smoothness. To do this, we first randomly select 100 users and 300 items from the original \emph{MovieLens} dataset, and get a \emph{MovieLens100} dataset, which consists 1576 ratings. We then use different smoothness objective function, i.e., the pairwise smoothness objective function shown in Eq.(\ref{pair}) and the joint smoothness objective function shown in Eq.(\ref{joint}), in our proposed model. The joint smoothness is described in Section \hyperref[sec-energyfunction]{\ref{sec-energyfunction}}, and we term it ``joint'' here for simplification. We also use two kinds of approaches to build the pairwise affinity graph: (1) $P_{ij,ko} = W_{ij} * S_{ko}$, and (2) $P_{ij,ko} = min\{W_{ij},S_{ko}\}$. We term these two pairwise approaches ``pairwise1'' and ``pairwise2'' respectively. We finally compare their runtime and prediction differences on \emph{MovieLens100}. The result is shown in Table \ref{smoothness-compare}, where we set $K=10$.  As we analyzed in Section \hyperref[pairwise-to-joint]{\ref{pairwise-to-joint}},  the runtime of joint smoothness is significantly shorter than pairwise smoothness. Besides, surprisingly, the performance of joint smoothness also significantly outperforms pairwise smoothness. We believe this is because joint smoothness simplifies the choice of $F_P(F_U,F_V)$, and the ways we used to build pairwise affinity graph is not good enough to represent the affinitive relationship between U-I pairs. We will leave how to build a good pairwise graph as our future work.

\begin{table}\scriptsize
\centering
\caption{Performance comparison between pairwise smoothness and joint smoothness.}
\label{smoothness-compare}
\begin{tabular}{|c|c|c|c|}
 \hline
  Metric & MAE & RMSE & runtime (seconds) \\
  \hline
  \hline
  pair1 & 1.4523 & 1.8412 & 2387 \\ 
  \hline
  pair2 & 1.4332 & 1.8221 & 935 \\ 
  \hline
  joint & \textbf{1.2613} & \textbf{1.5938} & \textbf{3}\\
  \hline
\end{tabular}
\vskip -0.00in
\end{table}

\subsection{Effect of Model Parameters}\label{parametereffect}

\begin{figure}
\centering
\subfigure [\emph{Precision@50}]{ \includegraphics[width=4cm]{figures/deliciousfg-precision}}
\subfigure[\emph{Recall@50}] { \includegraphics[width=4cm]{figures/deliciousfg}}
\vskip -0.15in
\caption{Effect of smoothness degree parameters $\lambda_F$ and $\lambda_G$ on RSCGM by setting $K=100$. Dataset used: \emph{Delicious}.}
\label{graphfg}
\vskip -0.05in
\end{figure}

\begin{figure}
\centering
\subfigure [\emph{Precision@50}]{ \includegraphics[width=3.9cm]{figures/lastfm-alpha-precision}}
\subfigure[\emph{Recall@50}] { \includegraphics[width=4.1cm]{figures/lastfm-alpha-recall}}
\vskip -0.15in
\caption{Effect of smoothness confidence decay parameters $\alpha$ on RSCGM. Dataset used: \emph{Lastfm}.}
\label{alpha}
\vskip -0.05in
\end{figure}

We first study the effect of the smoothness degree parameters, i.e., $\lambda_F$ and $\lambda_G$, on our model performance. By doing this, we set $\alpha=1$, $d=0$, and vary the values of $\lambda_F$ and $\lambda_G$ to see their effect on model performance. That is, we only propagate the known ratings to their direct neighbors. 
%Take Figure \ref{propagation} for example, we only propagate the rating of $R_{42}$ to its direct neighbors, i.e., $r_{32}$ and $4_{52}$.

Figure \ref{graphfg} shows the effect of $\lambda_F$ and $\lambda_G$ on RSCGM, where we set $k=100$ and $M=50$. We can see that RSCGM achieves the best \emph{Precision} and \emph{Recall} performance when $\lambda_F=\lambda_G=0.001$ on \emph{Delicious}.
The results indicate that smoothness on both user and item affinity graphs contribute to model performance, which proves the effectiveness of our joint-smoothness idea.

We then study the effect of the smoothness confidence decay parameter, i.e., $\alpha$, on our model performance. By doing this, we set $\lambda_F$ and $\lambda_G$ to the best values obtained using the above method. Figure \ref{graphfg} shows the effect of $\alpha$ on RSCGM, where we set $M=50$. From it, we can see that, with the increase of $\alpha$, the performance first increases, and then decreases after a certain threshold. The explanation is: (1) when $\alpha$ is small, with the increase of propagation length $d$, the local smoothness confidence $\alpha^{|d|+1}$ will be too small to propagate ratings. That is, known ratings will only be propagated to short path neighbors with a small $\alpha$, and this may cause information loss. (2) On the contrary, with a big $\alpha$, known ratings will be propagated to their long path neighbors, and this may cause data noise due to the unreliable affinity graphs in data sparsity scenario.


\subsection{Computation Time}

We run our model on a PC with 2.33 GHz Intel(R) Xeon(R) CPU and 8Gb RAM.
Figure \ref{time} shows the wall-clock running time per iteration of our proposed model with different size of training data on the \emph{Lastfm}, where we set $\alpha=0.3$ and $\alpha=0.4$ respectively. The same as we analyzed in Section \hyperref[parameter-learning]{\ref{parameter-learning}}, with the increase of $\alpha$, the runtime decrease, and the runtime increases linear with the observed data, no matter what is the value of $\alpha$.
Besides, further observation shows that, the bigger the dimensionality $K$ is, the bigger the runtime increase rate is. This is because the runtime can be seen as a linear function of the observed data size, and its slope is $(\sum{\overline{F}} + \sum{\overline{G}}) K$. With a relative stable value of $\sum{\overline{F}} + \sum{\overline{G}}$, the bigger $K$ is, the bigger the increase slope is.

\begin{figure}
\centering
\subfigure[$\alpha=0.3$] { \includegraphics[width=4cm]{figures/lastfm-runtime-3}}
\subfigure [\emph{$\alpha=0.4$}]{ \includegraphics[width=4cm]{figures/lastfm-runtime-4}}
\vskip -0.15in
\caption{Wall-clock time with different size of training data on \emph{Lastfm}.}
\label{time}
\vskip -0.1in
\end{figure}


==> section/sec-intro-20171218.tex <==

\section{Introduction}\label{intro}
As e-commerce platforms and online social networks provide customers and users myriad products and massive information, a \emph{recommender system} (RS) has become a useful and even indispensable facility for information filtering.
In fact, RS is now part of our daily activities, as it has been widely adopted by internet service leaders, such as Amazon, Youtube, and Facebook \cite{sarwar2001item}.

\stitle{Data sparsity challenge.}As \emph{users} have actions (e.g., rate and buy) on some \emph{items}, RS aims to predict the users' unknown actions on other items.
The tendency of a user's action on an item can be indicated by a real-valued number, i.e., \emph{rating} or \emph{label}. Thus, RS is also known as the \emph{unknown ratings prediction} problem \cite{shi2014collaborative}. 
In practice, however, many RSs have to evaluate very large user and item sets, where the user-item (U-I) matrix is extremely sparse-- such \emph{data sparsity} has always been the main challenge of RS \cite{su2009survey}.


%Given a user set $\mathds{U}=\{u_1,...,u_I\}$ and an item set $\mathds{V}=\{v_1,...,v_J\}$, where \emph{I} and \emph{J} denote the number of users and items.
%We use $\bm{R}$ to represent the user-item (U-I) rating matrix, with each element $R_{ij}$ denoting the rating that $u_i$ gives to $v_j$. In practice, $R_{ij}$ is often given as integers, such as in the range [1, 5] on MovieLens. We use $\bm{r}$ to represent the predicted U-I rating matrix, with a real-valued number $r_{ij}$ denoting the predicted rating of $u_i$ on $v_j$. There are totally $I \times J$ ratings, among which only $\mathscr{L}$ ratings are known, and our recommendation task is to predict the unknown ratings in $\bm{R}$, with the size of $\mathscr{U}=I \times J-\mathscr{L}$.

%\stitle{Data sparsity.}

So far, two techniques have been popularly used to alleviate the data sparsity problem of RS, i.e., \emph{semi-supervised learning} (SSL) and \emph{latent factor model} (LFM).

\stitle{Semi-supervised learning.}SSL uses unlabeled data to either modify or reprioritize hypotheses obtained from labeled data alone, and thus can alleviate the label 
sparsity problem \cite{seeger2000learning}. 
%Note that `rating' is called from the perspective of RS and `label' is called from that of SSL, and we use them interchangeably in this paper. 
Towards effective SSL, affinity graph-based smoothness approaches have attracted much research interests, which follow the \emph{smoothness} insight: \emph{close nodes on an affinity graph have similar labels}. 
%The affinity graph is used to capture the affinity between data. 
Graph-based SSL is appealing recently because it is easy to implement and gives rise to closed-form solutions \cite{zhu2003semi,chapelle2006semi,wang2006recommendation,ding2007learning,wang2010enhanced,fang2014graph}. 
%In a RS scenario, each data object $(u_i,v_j)$ is a U-I pair, with a rating $R_{ij}$ as its label, and thus, to adopt SSL for rating prediction in RS, rating smoothness should exist among U-I pairs.


\stitle{Latent factor model.}LFM increases the rating density by reducing the dimensionality of U-I rating matrix, and thus is able to alleviate the data sparsity problem.  
LFM uses a low dimensional user and item latent factors to represent the characteristics of each user and each item, and uses the product of them to represent the user's rating on the item. LFM has drawn much attention recently due to its good performance and scalability \cite{mnih2007probabilistic,koren2008factorization,takacs2008investigation,agarwal2009regression,rendle2010factorization,wang2011collaborative,purushotham2012collaborative,kanagal2013focused,xu2015ice,liu2016kernelized,guo2016novel,beutel2017beyond}.

Although SSL and LFM have their own merits to alleviate the data sparsity problem, they  have their own disadvantages. 
Graph-based SSL directly predicts the unknown ratings in the original U-I matrix, and thus suffers from the scalability problem. Meanwhile, LFM focuses on regressing the rare labelled data, and fails to capture the smoothness insight between ratings, unlike SSL, and thus its performance is further limited under data sparsity scenario \cite{agarwal2009regression}.

%LFM scales linearly with the labelled data size due to the use of dimensionality reduction technique \cite{koren2008factorization,agarwal2009regression,rendle2010factorization}, and thus can solve the scalability problem of SSL. 
%Because LFM predicts ratings by learning low dimensional user and item latent factors,  instead of predicting the ratings directly, which is the same reason as it solves the scalability problem of memory-based collaborative filtering approach \cite{su2009survey}.


As a key insight of this paper, we identify the marriage of SSL and LFM. 
The main insights of SSL (i.e., \emph{smoothness}) and LFM (i.e., \emph{dimensionality reduction}) are orthogonal, and they are likely to benefit from each other. However, surprisingly, the synergy between SSL and LFM has not been explored. 
On one hand, the smoothness idea of SSL, i.e., similar users or items should give or receive similar ratings-- across the entire U-I matrix of ratings, known or unknown, can mitigate the data sparsity problem of LFM. On the other hand, the dimensionality reduction idea of LFM can solve the scalability problem of SSL, since the prediction is done in a low rank matrix instead of the original high dimensional matrix. 
%We will analyze our model time complexity in Section \hyperref[parameter-learning]{\ref{parameter-learning}}.

\stitle{Challenges of marrying SSL with LFM.}However, marrying SSL with LFM to do recommendation is nontrivial. 
We summarize the main challenges as follows:
%Recently, there is an attempt of using the dimensionality reduction idea of LFM to realize the similar idea of SSL \cite{ma2011recommender,gu2010collaborative,chen2014context}. They assume that connected users or items on a graph tend to share similar user or item latent factors, which we term it ``\emph{latent factor restriction}'' (LFR) hereafter. That is, they capture the correlation dependency between latent factors, not ratings. We will explain in Section \hyperref[relatedwork-lfr]{\ref{relatedwork-lfr}} that they use an overly strong assumption which limits their performance, and experiments in Section \hyperref[experiments]{\ref{experiments}} will demonstrate their deficiency, especially in data sparsity scenarios. Moreover, several efforts have attempted to directly adopt SSL to do recommendation without using the dimensionality reduction idea of LFM  \cite{wang2006recommendation,ding2007learning,wang2010enhanced}. They first build a user or an item social network based on the rare user social relationships or ratings, and then perform rating propagation on them. They not only overlook that the networks are built based on the rare information and thus are unreliable, but also neglect the reality that the rating smoothness in a RS scenario should be between U-I pairs, instead of only users or items, as we described above.

\sstitle{Challenge $\mathcal{I}$: Disparate unification.}~SSL predicts unknown ratings through rating propagation on affinity graphs. I.e., SSL captures the correlation dependency between ratings. LFM predicts unknown ratings through learning user and item latent factors by regressing known ratings. I.e., LFM captures the causal dependency between latent factors and ratings. 
%Usually, a single model only has the ability to capture single dependency between variables, e.g., \cite{mnih2007probabilistic,koren2008factorization,agarwal2009regression,rendle2010factorization,wang2011collaborative}.
%Thus, how to build a unified model so that such different dependency between different variables can be captured is the first challenge.
Therefore, we aim to propose a principled framework to unify SSL and LFM so that such different dependency between different variables can be captured.

\sstitle{Challenge $\mathcal{II}$: Expensive graph construction.}~In a RS scenario, each data object $(u_i,v_j)$ is a U-I pair, with a rating $R_{ij}$ as its label, and thus, to adopt SSL for rating prediction in RS, rating smoothness should exist among U-I pairs.
%In a RS scenario, each data object is a U-I pair, e.g., $\{u_i,v_j\}$, with a rating as its label, e.g., $R_{ij}$, and thus, to adopt SSL for rating prediction in RS, we need to perform rating smoothness among U-I pairs. 
Suppose we have \emph{I} users and \emph{J} items, building such a U-I pairwise affinity graph needs to compute the similarity between each of $ I \times J$ U-I pairs, with a time complexity of $O{(I \times J)}^2$, and thus, cannot scale to large datasets. 
%Moreover, as described above, directly using graph-based SSL to do prediction needs a cubic time complexity $O(\mathscr{U}^3)$ where $\mathscr{U}$ is a very large.
%Thus how to find a smoothness approach which possesses low time complexity and similar performance with pairwise smoothness becomes the second challenge.
Thus, we aim to realize smoothness in a more efficient manner.

\sstitle{Challenge $\mathcal{III}$: Unreliable affinity.}~In a traditional SSL scenario, the affinity graphs are built based on the characteristics of the data itself, e.g., the pixel data of a scanned digit. In contrast, in a RS scenario, the affinity graphs are usually built based on user social relationships or ratings \cite{wang2006recommendation,ding2007learning,wang2010enhanced,purushotham2012collaborative,ma2011recommender,gu2010collaborative,chen2014context}. As a result, the affinity graphs are unreliable due to the sparsity of such user social relationships or ratings. 
Thus, we aim to alleviate the unreliable affinity problem in a robust way.
%How to perform rating propagation on an unreliable affinity graph is the third great challenge. 

\stitle{Our proposal: Learning to recommend with CGM.}Our proposal is based on the following insights.
%In this paper, we propose a novel chain graph model (CGM), which is a combination of Bayesian network and Markov random field, and is able to marry SSL and LFM successfully.
%which are based on the following insights:

\sstitle{Insight $\mathcal{I}$: Principled unification.}~To address Challenge $\mathcal{I}$, we propose a novel chain graph model (CGM) to marry SSL with LFM. As far as we know, this is the first attempt in the literature to adopt CGM in RS. A CGM is a combination of Bayesian network and Markov random field, which has the ability to capture different kinds of dependency (i.e., correlation and causal dependency) between different kinds of variables (i.e., latent factors and ratings) \cite{lauritzen2002chain,bishop2006pattern,mackey2007latent}. Thus, CGM is an ideal model to solve Challenge $\mathcal{I}$.

%we need a way that not only can capture different kinds of dependency (i.e., correlation dependency and causal dependency), but also is able to capture the dependency between different kinds of variables (i.e., latent factor and rating). 
%Bayesian network is commonly used to model the rating generation and regression from user and item latent factors \cite{mnih2007probabilistic,wang2011collaborative,purushotham2012collaborative}. Markov random field is commonly used to model the correlation dependency between variables \cite{domingos2001mining}. 
%As a combination of Bayesian network and Markov random field, 

\sstitle{Insight $\mathcal{II}$: Efficient smoothness.}~To address Challenge $\mathcal{II}$, we develop a novel ``joint smoothness'' framework to realize SSL on a pair of decomposed user and item affinity graphs.
%In the RS scenario, each data object is a U-I pair, and this results in Challenge $\mathcal{II}$. Although pairwise smoothness is a standard way to perform smoothness, it results in high time complexity. 
Since a rating is given from a user to an item, smoothness exists in two dimensions, i.e., user and item. We term it \emph{joint-smoothness}, which enables us to decrease the time complexity to build affinitive graphs to $O(I^2 + J^2)$. 
%Thus, joint-smoothness is a way to solve Challenge $\mathcal{II}$.

\sstitle{Insight $\mathcal{III}$: Selective smoothness.}~To address Challenge $\mathcal{III}$, we propose a confidence-aware smoothness approach. 
%To our knowledge, our effort is the first in the literature to identify the unreliable affinity  problem in RS and propose a solution.
Different from the traditional SSL which performs rating propagation (i.e., smoothness constraint) everywhere on the affinity graphs, we choose to perform smoothness selectively. 
Specifically, we propose a smoothness confidence decay model to control the hops of rating propagation length.%enables us to only propagate the known ratings to their close neighbors.
%Thus, a confidence-aware selective smoothness method is an effective way to solve Challenge $\mathcal{III}$.

\sstitle{Solutions.}~First, we propose a novel CGM (Section \hyperref[cfssl]{\ref{cfssl}}), which is a combination of Bayesian network and Markov random field.
%Our proposed CGM contains three layers. The first layer is the \emph{latent factor layer}. The second layer is the \emph{prediction layer}. The third layer is the \emph{observation layer}. From the latent factor layer to the prediction layer, it is the rating generation procedure. In the prediction layer, it is the prediction smoothness constraint of SSL. From the prediction layer to the observation layer, it is the rating regression objective of the existing LFMs. %, i.e., the predicted rating should be close to the observed rating. 
%We use Bayesian network to model the rating generation and regression procedures, and use Markov random field to model the rating smoothness constrain. 
Second, we propose a joint-smoothness objective function. Instead of building a U-I pairwise affinity graph, we build two decomposed user and item affinity graphs. 
%We first describe the derivation from pairwise to joint smoothness (Section \hyperref[pairwise-to-joint]{\ref{pairwise-to-joint}}), 
%and then present the affinity graphs build method (Section \hyperref[sec-energyfunction-buildgraph]{\ref{sec-energyfunction-buildgraph}}).
Third, we propose a confidence-aware smoothness approach (Section \hyperref[confident-pairwise-to-joint]{\ref{confident-pairwise-to-joint}}). This selective smoothness approach not only alleviates the graph unreliable problem in RS scenarios, but also saves huge computation. 
%The dimensionality idea of LFM and the confidence-aware smoothness idea will make our model scales linear with the observed data size.
Finally, we present the model learning method based on coordinate descent (Section \hyperref[parameter-learning]{\ref{parameter-learning}}).

%Specifically, we build two undirected user and item decomposed affinity graphs, i.e., Markov random fields, to represent the affinitive relationship between users and items. Finally, the posterior distribution over the user and item latent factors can be obtained through Bayesian theory, and then it can be solved by using coordinate descent. Getting user and item latent factors will enable us to predict any unknown U-I rating pairs.

%we propose a confidence-based joint-smoothness energy function to model the probability of smoothness relationship between the generated U-I ratings pairs on user and item affinity graphs (Section V). That is, we use Markov random field to model the smoothness constrain between the generated ratings on the user and item affinity graphs. However, different from the traditional SSL that performs rating propagation (i.e., smoothness constrain) everywhere on the affinity graphs, we only propagate the known ratings to their close neighbors, where we have strong confidence. By doing this, we are able to not only alleviate the graph unreliable problem in RS scenario, but also save huge computation.

%Our proposed chain graph model realizes the idea of both SSL and LFM, and thus possesses the merits of both of them. On one hand, the data sparsity issue of LFMs is alleviated by using the smoothness idea of SSL. One the other hand, the scalability problem of SSL is solved by using the dimensionality reduction technique of LFMs.

\sstitle{Results.}~We concretely realize our solutions of marrying SSL with two kinds of popular LFMs, and conduct comprehensive experiments in Section \hyperref[experiments]{\ref{experiments}}. Our experiments are conducted on \emph{three} popular datasets, with \emph{nine} state-of-the-art comparison approaches. We use \emph{four} metrics to evaluate model performance. The experimental results show that our approach significantly outperforms the state-of-the-art methods, especially in data sparsity scenarios.

\stitle{Contributions.}We summarize the main contributions in this paper as follows: 
\begin{itemize}[leftmargin=*] \setlength{\itemsep}{-\itemsep}
    \item We propose a novel CGM to marry SSL with LFM for alleviating the data sparsity problem of RS, which we believe is the first attempt in the literature.
    \item We propose to perform joint-smoothness instead of pairwise smoothness, which has better efficiency.
    \item We propose a confidence-aware smoothness approach to alleviate the unreliable graph problem in RS scenario. To the best of our knowledge, it is also the first attempt.
   \item Our model scales linearly with the observed data size, since we adopt dimensionality reduction technique and confidence-aware smoothness approach.
\end{itemize}


%(1) We propose a novel CGM to marry SSL and LFM for alleviating the data sparsity problem of RS, and we also present the model learning methods using coordinate descent (Section \hyperref[parameter-learning]{\ref{parameter-learning}}). As far as we know, this is the first attempt in the literature to adopt CGM in RS; (2) We propose to perform joint-smoothness instead of pairwise smoothness; (3) We propose a confidence-aware joint-smoothness energy function to alleviate the graph unreliable problem in RS scenario. To the best of our knowledge, it is the first attempt in the literature to identify the affinity unreliable problem in RS and propose an approach to solve it; (4) Our models can be applied to very large datasets since it scales linearly with the total number of observed data.

The rest of the paper is organized as follows. In Section \hyperref[relatedwork]{\ref{relatedwork}}, we review related work. 
In Section \hyperref[preliminary]{\ref{preliminary}}, we describe the popular realizations of SSL and LFM. 
In Section \hyperref[cfssl]{\ref{cfssl}}, we propose a novel probabilistic CGM to marry SSL with LFM.
In Section \hyperref[cfssl]{\ref{cfssl}}, we present the confidence-aware joint-smoothness energy function.
In Section \hyperref[parameter-learning]{\ref{parameter-learning}}, we present the model learning approach based on gradient descent. 
In Section \hyperref[experiments]{\ref{experiments}}, we present the experimental results and analysis. 
Finally, we conclude the paper in Section \hyperref[conclusion]{\ref{conclusion}}.

